Exploring the robust extrapolation of high-dimensional machine learning potentials

We show that, contrary to popular assumptions, predictions from machine learning potentials built upon high-dimensional atom-density representations almost exclusively occur in regions of the representation space which lie outside the convex hull defined by the training set points. We then propose a perspective to rationalize the domain of robust extrapolation and accurate prediction of atomistic machine learning potentials in terms of the probability density induced by training points in the representation space

==> SM_prb/defs.tex <==
\input{dirac-rep}
\newcommand{\vv}[1]{\bm{#1}}
\newcommand{\strg}[1]{\mathrm{#1}}
\newcommand{\crl}[1]{\mathcal{#1}}

\newcommand{\density}[3]{ \braket*{#1}{#2}_{#3} }
\newcommand{\densitydag}[3]{  \braket*{#2}{#1}_{#3} }
\newcommand{\densitym}[4]{ \matrixel{#1}{#4}{#2}_{#3} }
\newcommand{\densitysqt}[3]{ \braket*{#1}{#2^{(2)}}_{#3} }
\newcommand{\densitysq}[3]{ \braket{#1}{#2^{(1)}}_{#3} }
\newcommand{\densitysqdag}[3]{  \braket{#2^{(1)}}{#1}_{#3} }
\newcommand{\densitycube}[3]{ \braket*{#1}{#2^{(2)}}_{#3} }

\newcommand{\smearing}[1]{g\left(#1\right)}
\newcommand{\gaus}[2]{\CN_{#2}\pqty\big{#1}}
\newcommand{\ddelta}[1]{\delta(#1)}

\newcommand{\xj}{\mathcal{X}_{j}}
\newcommand{\xk}{\mathcal{X}_{k}}
\newcommand{\bri}{\mathbf{r}_i}
\newcommand{\brj}{\mathbf{r}_j}
\newcommand{\brij}{\mathbf{r}_{ij}}

\newcommand{\bu}{\mathbf{u}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\That}{\hat{t}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\bPsi}{\mathbf{\Psi}}
\newcommand{\bPhi}{\mathbf{\Phi}}
\newcommand{\dint}{\textrm{d}}
\newcommand{\dbr}{\dint\br}
\newcommand{\dThat}{\dint\That}
\newcommand{\dRhat}{\dint\Rhat}
\newcommand{\drhat}{\dint\brhat}
\newcommand{\cald}{\mathcal{D}}
\newcommand{\calk}{\mathcal{K}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\loss}{\ell}
\newcommand{\diag}{\ensuremath{\operatorname{diag}}}
\newcommand{\iket}[2]{\ket{#1}_{#2}}
\newcommand{\ibraket}[3]{\braket{#1}{#2}_{#3}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\sothree}{\ensuremath{\mathcal{SO}\left(3\right)}}
\newcommand{\othree}{\ensuremath{{\mathcal{O}\left(3\right)}}}
\newcommand{\behat}{\ensuremath{\hat{\mathbf{e}}}}
\newcommand{\angstrom}{\text{\AA}}

\newcommand{\D}[1]{\operatorname{d}{#1}} 
\newcommand{\gs}{\ensuremath{g_\text{s}}}
\newcommand{\gb}{\ensuremath{g_\text{b}}}
\newcommand{\nmax}{\ensuremath{n_\text{max}}}
\newcommand{\lmax}{\ensuremath{l_\text{max}}}

\newcommand{\DOS}{\mathrm{DOS}}
\newcommand{\LDOS}{\mathrm{LDOS}}
\newcommand{\LADOS}{\mathrm{LADOS}}
\newcommand{\Eband}{\epsilon_{\text{band}}}
\newcommand{\Efermi}{\epsilon_{F}}


==> SM_prb/dirac-rep.tex <==
\usepackage{physics}
\usepackage{xparse}

% shortcuts for boldface and calligraphic
\newcommand{\mcal}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\mbf}[1]{\ensuremath{\mathbf{#1}}}

% a macro to typeset representations in bra-ket notation.
% can be used either with just ket \rep|A> or bra \rep<X|
% or together, \rep <X||A>
\NewDocumentCommand{\rep}{s d<| d|>}{%
% flips starring behavior relative to physics package 
\IfBooleanTF{#1}{
   \IfValueTF{#2}{
       \IfValueTF{#3}{\braket{#2}{#3}}{\bra{#2}}
       }{
       \IfValueTF{#3}{\ket{#3}}{}
       }
   }{
   \IfValueTF{#2}{
       \IfValueTF{#3}{\braket*{#2}{#3}}{\bra*{#2}}
       }{
       \IfValueTF{#3}{\ket*{#3}}{}
       }
   }
}

% for those who prefer the physics package \bra \ket notation
\NewDocumentCommand{\rbra}{sm}{\IfBooleanTF{#1}{\rep*<#2|}{\rep<#2|}}
\NewDocumentCommand{\rket}{sm}{\IfBooleanTF{#1}{\rep*|#2>}{\rep|#2>}}
\NewDocumentCommand{\rbraket}{smm}{\IfBooleanTF{#1}{\rep*<#2||#3>}{\rep<#2||#3>}}

% shortcut for CG "our way"
\NewDocumentCommand{\cg}{m m m}{\rep<#1; #2||#3>}

% macro to typeset a field. very flexible, should allow
% to describe non-symmetrized fields \field{\rho}
% fields that are symmetrized just once \field{\rho}x{\nu}
% equivariant fields \field[lambda mu]{\rho}x2
% and multi-scale LODE \field{\rho}x{\nu}[V]x{\nu'}
\NewDocumentCommand{\field}{o m e{_} e{^} o e{_} e{^}}{
% use overline if an otimes argument is specified, or if there is a double field entry
\IfValueTF{#5}{\overline{
  #2\IfValueT{#3}{_#3}\IfValueT{#4}{^{\otimes #4}} % first block
  \otimes 
  #5\IfValueT{#6}{_#6}\IfValueT{#7}{^{\otimes #7}} % second block
  \IfValueT{#1}{;#1}
}}{
  \IfValueTF{#4}{\overline{
     #2\IfValueT{#3}{_#3}\IfValueT{#4}{^{\otimes #4}}
     \IfValueT{#1}{;#1}
  }}
  {#2\IfValueT{#3}{_#3}}
}
}

% shortcuts for commonly-used fields
\NewDocumentCommand{\frho}{o e{_} e{^}}{
\field[#1]{\rho}_{#2}^{#3}
}

% shortcuts for commonly used feature indices

\newcommand{\e}{a}  % element index

% we use \bx for Cartesian basis, and \br to indicate atom positions
\newcommand{\br}{\mbf{r}}
\newcommand{\bx}{\mbf{x}}
\newcommand{\bxhat}{\hat{\mbf{x}}}
\newcommand{\brhat}{\hat{\mbf{r}}}

\NewDocumentCommand{\ex}{e_}{
\IfValueTF{#1}{\e_{#1}\bx_{#1}}{\e\bx}
}  % element index

% common indices for fully discretized density basis, and all sorts of combinations of subindices
\NewDocumentCommand{\lm}{e_}{
\IfValueTF{#1}{l_{#1}m_{#1}}{lm}
}
\NewDocumentCommand{\nlm}{e_}{
\IfValueTF{#1}{n_{#1}\lm_{#1}}{n\lm}
}
\NewDocumentCommand{\enlm}{e_}{
\IfValueTF{#1}{\e_{#1}\nlm_{#1}}{\e\nlm}
}
\NewDocumentCommand{\en}{e_}{
\IfValueTF{#1}{\e_{#1}n_{#1}}{\e n}
}
% coupled angular momentum basis
\NewDocumentCommand{\nlk}{e_}{
\IfValueTF{#1}{n_{#1}l_{#1}k_{#1}}{nlk}
}
\NewDocumentCommand{\enlk}{e_}{
\IfValueTF{#1}{\e_{#1}\nlk_{#1}}{\e\nlk}
}
\NewDocumentCommand{\enl}{e_}{
\IfValueTF{#1}{\en_{#1}l_#1}{\en l}
}
\NewDocumentCommand{\nl}{e_}{
\IfValueTF{#1}{n_{#1}l_#1}{n l}
}

% SOAP shortcuts - starred version removes ; separators
\NewDocumentCommand{\nnl}{s}{
\IfBooleanTF{#1}{n_1 n_2 l}{n_1; n_2; l}
}
\NewDocumentCommand{\ennl}{s}{
\IfBooleanTF{#1}{\en_1 \en_2 l}{\en_1; \en_2; l}
}

% greek indices for equivariants
\NewDocumentCommand{\gslm}{s}{
\IfBooleanTF{#1}{\sigma\lambda\mu}{\sigma;\lambda\mu}
}
\NewDocumentCommand{\glm}{}{\lambda\mu}
